Benefits of Overparameterized Convolutional Residual Networks: Function Approximation under Smoothness Constraint

Overparameterized neural networks enjoy great representation power on complex data, and more importantly yield sufficiently smooth output, which is crucial to their generalization and robustness. Most existing function approximation theories suggest that with sufficiently many parameters, neural networks can well approximate certain classes of functions in terms of the function value. The neural network themselves, however, can be highly nonsmooth. To bridge this gap, we take convolutional residual networks (ConvResNets) as an example, and prove that large ConvResNets can not only approximate a target function in terms of function value, but also exhibit sufficient first-order smoothness. Moreover, we extend our theory to approximating functions supported on a low-dimensional manifold. Our theory partially justifies the benefits of using deep and wide networks in practice. Numerical experiments on adversarial robust image classification are provided to support our theory.

==> mainproof.tex <==
\section{Proof of Theorem \ref{thm.D}}
\label{sec.proof.D}
\begin{proof}[Proof of Theorem \ref{thm.D}]
	We prove Theorem \ref{thm.D} in four steps.
	%The proof of Theorem \ref{thm.D} is similar to that of \citet[Theorem 4.1]{guhring2020error}.
	\paragraph{Step 1: Decompose $(0,1)^D$ using locally supported functions.} We define 
	\begin{align}
		\psi(x)=\begin{cases}
			1 & |x|<1,\\
			0 & 2<|x|,\\
			2-|x| & 1\leq |x|\leq 2
		\end{cases}
	\end{align}
	and 
	\begin{align}
		\phi_{\mb}(\xb)=\prod_{k=1}^D \psi\left(3N\left(x_k-\frac{m_k}{N}\right)\right)
	\end{align}
	with $\mb=(m_1,m_2,...,m_D)\in \{0,...,N\}^D$. We have $\sum_{\mb} \phi_{\mb}=1$ on $(0,1)^D$ and $\phi_{\mb}$ is supported on $B_{\frac{2}{3}N,\|\cdot\|_{\infty}}(\frac{\mb}{N})\subset B_{1/N,\|\cdot\|_{\infty}}(\frac{\mb}{N})$. We denote $\cS_N=\{0,1,...,N\}^D$. The following lemma shows that each $\psi\left(3N\left(x_k-\frac{m_k}{N}\right)\right)$ can be realized by a CNN (see a proof in Appendix \ref{sec.psi}).
	\begin{lemma}\label{lem.psi}
		There exists a CNN architecture $\cF^{\rm CNN}(L,J,K,\kappa_1,\kappa_2)$ such that for any $N,m$, such an architecture yields a CNN $\widetilde{\psi}$ with
		\begin{align}
			&\widetilde{\psi}_{m,N}(x)=\psi\left(3N\left(x_k-\frac{m}{N}\right)\right), \label{eq.psi.CNN}\\
			&\|\widetilde{\psi}_{m,N}\|_{W^{k,\infty}(0,1)}\leq (3N)^k.
			\label{eq.psi.sobolev}
		\end{align}
		Such an architecture has
		$$
		L=2, \ J=16, \  K=2, \ \kappa_1=\kappa_2=O(N).
		$$
		Further more, the weight matrix in the fully connected layer of $\cF^{\rm CNN}$ has nonzero entries only in the first row.
	\end{lemma}
	We then decompose $f$ as
	\begin{align}
		f=\sum_{\mb} \phi_{\mb}f.
	\end{align}
	
	%\begin{lemma}
	%	For $k=0,1$, we have 
	%	$$
	%	\|\phi_{\mb}\|_{W^{k,\infty}(\RR^D)}\leq CN^k ,
	%	$$
	%	where $C$ is a constant.
	%\end{lemma}
	
	\paragraph{Step 2: Approximate each $\phi_{\mb}f$ using averaged Taylor polynomials.}
	On each $B_{1/N,\|\cdot\|_{\infty}}(\frac{\mb}{N})$, we approximate $\phi_{\mb}f$ by an averaged Taylor polynomial. The averaged Taylor polynomial is defined as follows
	\begin{definition}[Averaged Taylor polynomials]
		Let $\alpha>0, 1\leq p\leq +\infty$ be integers and $f\in W^{\alpha-1,p}(\Omega)$. For $\xb_0\in \Omega, r>0$ such that $\overline{B_{r,\|\cdot\|}(\xb_0)}$ is compact in $\Omega$, the corresponding Taylor polynomial of order $\alpha$ of $f$ averaged over $B_{r,\|\cdot\|}(\xb_0)$ is defined as
		\begin{align}
			Q_{\xb_0}^{\alpha}f(\xb)=\int_{B_{r,\|\cdot\|}(\xb_0)} T^{\alpha}f(\xb,\zb)\phi(\zb)d\zb
		\end{align}
		with
		\begin{align}
			T^{\alpha}f(\xb,\yb)=\sum_{|\vb|\leq \alpha-1} \frac{1}{\vb\!} \partial^{\vb}f(\zb)(\xb-\zb)^{\vb}
		\end{align}
		and $\phi$ being arbitrary cut-off function satisfying
		\begin{align*}
			&\phi\in C_c^{\infty}(\RR^D) \mbox{ with } \phi(\xb)\geq 0 \mbox{ for all } \xb\in \RR^D, \nonumber\\
			&\supp(\phi)=\overline{B_{r,\|\cdot\|}(\xb_0)} \mbox{ and } \int_{\RR^D}\phi(\xb)d\xb=1,
		\end{align*}
		where $C_c^{\infty}(\RR^D)$ denotes the space of infinitely differentiable functions on $\RR^D$ with compact support.
	\end{definition}
	Under proper assumptions, the averaged Taylor polynomial can approximate $f$ and its partial derivatives well. We first define the star-shaped sets and chunkiness parameter, which are used in the error estimation result.
	\begin{definition}[Star-shaped sets, Definition 4.2.2 of \cite{brenner2008mathematical}]\label{def.starshape}
		Let $\Omega,\widetilde{\Omega}\subset \RR^D$. Then $\Omega$ is called star-shaped with respect to $\widetilde{\Omega}$ if for all $\xb\in\Omega$, we have
		\begin{align*}
			\overline{\convex(\{\xb\}\cup \widetilde{\Omega})}\subset \Omega.
		\end{align*}
	\end{definition}
	
	\begin{definition}[Chunkiness parameter, Definition 4.2.16 of \cite{brenner2008mathematical}]\label{def.chunkiness}
		Let $\Omega\subset\RR^D$ be bounded. Define
		\begin{align*}
			\cR=\big\{ &r>0: \mbox{ there exists } \xb\in \Omega \mbox{ such that } \\
			&\Omega \mbox{ is star-shaped with respect to } B_{r,|\cdot|}(\xb) \big\}.
		\end{align*}
		
		For $\cR\neq \emptyset$, we define
		$$
		r_{\max}^*=\sup \cR \quad  \mbox{ and } \quad \gamma=\frac{\diam(\Omega)}{r_{\max}^*},
		$$
		where $\gamma$ is called the chunkiness parameter of $\Omega$.
	\end{definition}
	The following lemma gives an error estimation of averaged Taylor polynomials:
	\begin{lemma}[Bramble-Hilbert, Lemma 4.3.8 of \cite{brenner2008mathematical}]
		\label{lem.ATE.error}
		Let $\Omega\subset \RR^D$ be open and bounded, $\xb\in \Omega$ and $r>0$ such that $\Omega$ is star-shaped with respect to $B_{r,\|\cdot\|}(\xb_0)$ and $r>\frac{1}{2} r^*_{\max}$, with $r^*_{\max}$ defined in Definition \ref{def.chunkiness}. Let $n>0,1\leq p \leq +\infty$ be integers and $\gamma$ be the chunkiness parameter of $\Omega$. Then we have
		\begin{align}
			|f-Q^{\alpha}_{\xb_0}f|_{W^{\alpha,p}(\Omega)}\leq Ch^{\alpha-k}|f|_{W^{\alpha,p}(\Omega)}
		\end{align}
		for $k=0,1,...,\alpha$, where $h=\diam(\Omega)$ and $C$ is a constant depending on $D,\alpha,\gamma$.
	\end{lemma}
	Lemma \ref{lem.aveTaylor.err} below shows that $Q^{\alpha}f$ can be written as a weighted sum of polynomials.
	\begin{lemma}[Lemma B.9 of \cite{guhring2020error}]\label{lem.aveTaylor.err}
		Let $\alpha>0, 1\leq p\leq +\infty$ be integers and $f\in W^{\alpha-1,p}(\Omega)$. Let $\xb_0\in\Omega, r>0$ such that $\overline{B_{r,\|\cdot\|}(\xb_0)}$ is compact in $\Omega$, and there exists $\widetilde{r}>0$ with  $B_{r,\|\cdot\|}(\xb_0)\subset B_{\widetilde{r},\|\cdot\|_{\infty}}(0)$. Then the averaged Taylor polynomial $Q_{\xb_0}^{\alpha}(f)$ can be written as
		\begin{align}
			Q_{\xb_0}^{\alpha}f(\xb)=\sum_{|\vb|\leq \alpha-1} c_{\vb}\xb^{\vb}
			\label{eq.aveTayloer.poly}
		\end{align}
		for $\xb\in \Omega$. There exists a constant $C$ depending on $\alpha,D,\widetilde{r}$ such that 
		$$
		|c_{\vb}|\leq Cr^{-D/p}\|f\|_{W^{\alpha-1,p}}(\Omega)
		$$
		for all $|\vb|\leq \alpha-1$.
	\end{lemma}
	
	Using averaged Taylor polynomials, we approximate $\phi_{\mb}f$ by
	\begin{align}
		\phi_{\mb}f\approx (\phi_{\mb}Q_{\mb/N}^{\alpha}f)(\xb)&=\phi_{\mb}\sum_{|\vb|\leq \alpha-1} c_{\mb,\vb}\xb^{\vb} \nonumber\\
		&=\sum_{|\vb|\leq \alpha-1} c_{\mb,\vb}\phi_{\mb}\xb^{\vb}.	
		\label{eq.f.aveTaylor}
	\end{align}
	Define 
	\begin{align}
		\widehat{f}=\sum_{\mb\in S_N}\sum_{|\vb|\leq \alpha-1} c_{\mb,\vb}\phi_{\mb}\xb^{\vb},
		\label{eq.f.aveTaylor1}
	\end{align}
	where $c_{\mb,\vb}$'s are the coefficients in (\ref{eq.aveTayloer.poly}).
	Then $\widehat{f}$ is an approximation of $f$. The following lemma gives an upper bound on the approximation error
	\begin{lemma}[Lemma C.4 of \cite{guhring2020error}]
		\label{lem.ATE.approx.error}
		Let $\alpha\geq 2$ be an integer and $1\leq p\leq \infty$. For any $s\in[0,1]$ and $f\in W^{\alpha,p}((0,1)^D)$, one has
		\begin{align}
			\|\widehat{f}-f\|_{W^{s,p}((0,1)^D)}\leq C\left( \frac{1}{N}\right)^{\alpha-s}\|f\|_{W^{\alpha,p}((0,1)^D)},
		\end{align}
		where $C$ is a constant depending on $\alpha,p,D$. Furthermore, the coefficients in $\widehat{f}$ satisfies
		\begin{align}
			|c_{\mb,\vb}|\leq C_1N^{D/p}\|f\|_{W^{\alpha,p}((0,1)^D)}
		\end{align} 
		for some constant $C_1$ depending on $D,\alpha,p$.
	\end{lemma}
	
	\paragraph{Step 3: Network approximation}
	Note that $\widehat{f}$ is a sum of functions in the form of $\phi_{\mb}\xb^{\vb}$ with weights $c_{\mb,\vb}$'s. We next approximate each $\phi_{\mb}\xb^{\vb}$ by a CNN.
	
	\begin{lemma}\label{lem.product}
		For any $0<\varepsilon<1, \xb\in (0,1)^D, N>0, \mb\in \{0,1,...,N\}^D,|\vb|<\alpha$, there exists a CNN architecture $\cF^{\rm CNN}(L,J,K,\kappa,\kappa)$ that yields a CNN $\widetilde{g}$ with
		\begin{align}
			&\|\widetilde{g}_{\mb,\vb}(\xb)-\phi_{\mb}\xb^{\vb}\|_{W^{k,\infty}((0,1)^D}\leq CN^k\varepsilon,
			\label{eq.product}\\
			&\widetilde{g}_{\mb,\vb}(\xb)=0 \mbox{ if } \phi_{\mb}\xb^{\vb}=0
			\label{eq.product0}
		\end{align}
		for $k=0,1$, where $C$ is a constant depending on $\alpha,k$. Such an architecture has
		\begin{align}
			L=O\left(D\log \frac{1}{\varepsilon}\right),\ J=O(D),\ \kappa=3N.
		\end{align}
		The constants hidden in $O$ depends on $\alpha,k$. 	Further more, the weight matrix in the fully connected layer of $\cF^{\rm CNN}$ has nonzero entries only in the first row.
	\end{lemma}
	Lemma \ref{lem.product} is proved in Appendix \ref{sec.product}. By Lemma \ref{lem.product}, each $\phi_{\mb}\xb^{\vb}$ can be approximated by a CNN. Denote the network approximation of $\phi_{\mb}\xb^{\vb}$ by $\widetilde{g}_{\mb,\vb}(\xb)$. We approximate $\widehat{f}$ by $\widetilde{f}$ defined as
	\begin{align}
		\widetilde{f}=\sum_{\mb} \sum_{|\vb|\leq \alpha-1} c_{\mb,\vb}\widetilde{g}_{\mb,\vb}(\xb).
		\label{eq.ftilde}
	\end{align}
	
	
	The following lemma gives an upper bound of the approximation error of $\widetilde{f}$ (see a proof in Appendix \ref{sec.net.error}).
	\begin{lemma}
		\label{lem.net.error}
		Let $\alpha\geq 2$ and $1\leq p\leq \infty$ be integers.
		For any $f\in W^{\alpha,p}((0,1)^D)$, let $\phi_{\mb}Q_{\mb/N}^{\alpha}f(\xb)$ be the averaged Taylor approximation of $\phi_{\mb}f$ defined in (\ref{eq.f.aveTaylor}). For any $0<\eta<1$, let $\widetilde{g}_{\mb,\vb}$ be the CNN approximation of $\phi_{\mb}Q_{\mb/N}^{\alpha}f(\xb)$ constructed in Lemma \ref{lem.product} with accuracy $\eta$.
		For $0\leq s \leq 1$, we have
		\begin{align}
			&\|\sum_{\mb\in \cS_N} \phi_{\mb}Q_{\mb/N}^{\alpha}f-\sum_{\mb\in \cS_N} \sum_{|\vb|\leq \alpha-1}c_{\mb,\vb}\widetilde{g}_{\mb,\vb}\|_{W^{s,p}((0,1)^D)} \nonumber\\
			&\leq C\|f\|_{W^{\alpha,p}((0,1)^D)}N^s\eta,
			\label{eq.neterr}
		\end{align}
		where $c_{\mb,\vb}$'s are coefficients defined in (\ref{eq.f.aveTaylor}), $C$ is a constant depending on $D,\alpha,s,p$.
	\end{lemma}
	Note the $\widetilde{f}$ is the sum of no more than $N^D(D+1)^{\alpha-1}$ CNNs of which the width is of $J=O(D)$. The following lemma shows that under appropriate conditions, the sum of $n_0$ CNNs with width in the same order can be realized by the sum of $n_1$ CNNs with a proper width (see a proof in Appendix \ref{sec.CNN.adap}):
	\begin{lemma}\label{lem.CNN.adap}
		Let $\{f_i\}_{i=1}^{n_0}$ be a set of CNNs with architecture $\cF^{\rm CNN}(L_0,J_0,K_0,\kappa_0,\kappa_0)$. For any integers $1\leq n\leq n_0$ and $\widetilde{J}$ satisfying $n\widetilde{J}=O(n_0)$ and $\widetilde{J}\geq J_0$, there exists a CNN architecture $\cF^{\rm CNN}(L,J,K,\kappa,\kappa)$ that gives a set of CNNs $\{g_i\}_{i=1}^{n}$  such that 
		\begin{align}
			\sum_{i=1}^{n} g_i(\xb)= \sum_{i=1}^{n_0} f_i(\xb).
		\end{align}
		Such an architecture has 
		\begin{align}
			L=O(L_0), J=O(\widetilde{J}), K=K_0, \kappa=\kappa_0.
		\end{align}
		Furthermore, the fully connected layer of $f$ has nonzero elements only in the first row.
	\end{lemma}
	
	
	
	By Lemma \ref{lem.CNN.adap}, for any $\widetilde{M},\widetilde{J}$ satisfying $\widetilde{M}\widetilde{J}=O(N^D)$, there exists a CNN architecture $\cF^{\rm CNN}(L,J,K,\kappa,\kappa)$ that gives rise to $\{g_i\}_{i=1}^n$ with 
	\begin{align*}
		\widetilde{f}=\sum_{i=1}^{\widetilde{M}} g_i,
	\end{align*}
	where
	\begin{align}
		L=O\left(\log \frac{1}{\eta}\right),\ J=O(\widetilde{J}),\ \kappa=3N.
	\end{align}
	
	The following lemma shows that the sum of CNNs can be realized by a ConvResNet:
	\begin{lemma}[Lemma 18 in \cite{liu2021besov}]\label{lem.cnn.convresnet}
		Let $\cF^{\rm CNN}(L,J,K,\kappa_1,\kappa_2)$ be any CNN architecture from $\RR^D$ to $\RR$. Assume the weight matrix in the fully connected layer of $\cF^{\rm CNN}(L,J,K,\kappa_1,\kappa_2)$ has nonzero entries only in the first row. Let $M$ be a positive integer. There exists a ConvResNet architecture $\cC(M,L,J,\kappa_1, \kappa_2(1\vee \kappa_1^{-1}))$ such that for any $\{f_i(\xb)\}_{i=1}^M\subset\cF^{\rm CNN}(L,J,K,\kappa_1,\kappa_2) $, there exists $\widetilde{f}\in \cC(M,L,J,\kappa_1, \kappa_2(1\vee \kappa_1^{-1}))$ with
		$$
		\widetilde{f}(\xb)=\sum_{i=1}^M f_i(\xb).
		$$
	\end{lemma}
	By Lemma \ref{lem.cnn.convresnet}, there exits a ConvResNet architecture  $\cC(M,L,J,K,\kappa_1,\kappa_2)$ with
	\begin{align}
		&L=O(\log 1/\eta), J=O(\widetilde{J}), \kappa_1=O(3N), \nonumber\\
		&\kappa_2=O(3N), M=O(\widetilde{M})
		\label{eq.net.para.1}
	\end{align}
	and $\widetilde{J},\widetilde{M}$ satisfying
	\begin{align}
		\widetilde{M}\widetilde{J}=O(N^D),
		\label{eq.net.para.2}
	\end{align}
	that yields a ConvResNet realizing $\widetilde{f}$.
	
	
	\paragraph{Step 4: Error estimation.} We compute
	\begin{align}
		&\|f-\widetilde{f}\|_{W^{s,p}((0,1)^D)} \nonumber\\
		\leq &\left\|f-\left(\sum_{\mb} \phi_{\mb}Q_{\mb/N}^{\alpha}f\right)\right\|_{W^{s,p}((0,1)^D)} \nonumber\\
		&+\left\|\left(\sum_{\mb} \phi_{\mb}Q_{\mb/N}^{\alpha}f\right)-\widetilde{f}\right\|_{W^{s,p}((0,1)^D)} \nonumber\\
		\leq &C_4\left( \frac{1}{N}\right)^{\alpha-s}\|f\|_{W^{\alpha,p}((0,1)^D)}+ C_5N^{s}\eta \|f\|_{W^{\alpha,p}((0,1)^D)} \nonumber\\
		\leq & (C_4+C_5)N^{-(\alpha-s)},
		\label{eq.neterror}
	\end{align}
	where $C_4,C_5$ are two constants depending on $D,\alpha,s,p,R$. In the second inequality, we use Lemma \ref{lem.ATE.approx.error} and \ref{lem.net.error} for the first and second term, respectively. In the third inequality, we set $\eta=N^{-\alpha}$ to balance the two terms. Using the relation (\ref{eq.net.para.2}), we have 
	\begin{align}
		N=(\widetilde{M}\widetilde{J})^{1/D}, \quad \eta=(\widetilde{M}\widetilde{J})^{-\frac{\alpha}{D}}.
		\label{eq.net.para.3}
	\end{align}
	
	Substituting (\ref{eq.net.para.3}) into (\ref{eq.neterror}) gives rise to 
	\begin{align}
		\|f-\widetilde{f}\|_{W^{s,p}((0,1)^D)}\leq C_6(\widetilde{M}\widetilde{J})^{-\frac{\alpha-s}{D}}
		\label{eq.neterror.1}
	\end{align}
	for some constant $C_6$ depending on $D,\alpha,s,p,R$.
	Substituting (\ref{eq.net.para.3}) into (\ref{eq.net.para.1}) and (\ref{eq.net.para.2}) gives rise to the network architecture
	\begin{align}
		&L=O(\log (\widetilde{M}\widetilde{J})), J=O(\widetilde{J}), \kappa_1=O((\widetilde{M}\widetilde{J})^{1/D}), \nonumber\\
		&\kappa_2=O((\widetilde{M}\widetilde{J})^{1/D}), M=O(\widetilde{M}).
	\end{align}
\end{proof}
